Toward Student-Oriented Teacher Network Training For Knowledge Distillation

How to conduct teacher training for knowledge distillation is still an open problem. It has been widely observed that a best-performing teacher does not necessarily yield the best-performing student, suggesting a fundamental discrepancy between the current teacher training practice and the ideal teacher training strategy. To fill this gap, we explore the feasibility of training a teacher that is oriented toward student performance with empirical risk minimization (ERM). Our analyses are inspired by the recent findings that the effectiveness of knowledge distillation hinges on the teacher's capability to approximate the true label distribution of training inputs. We theoretically establish that the ERM minimizer can approximate the true label distribution of training data as long as the feature extractor of the learner network is Lipschitz continuous and is robust to feature transformations. In light of our theory, we propose a teacher training method SoTeacher which incorporates Lipschitz regularization and consistency regularization into ERM. Experiments on benchmark datasets using various knowledge distillation algorithms and teacher-student pairs confirm that SoTeacher can improve student accuracy consistently.

==> inputs/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    % \answerTODO{}
    \answerYes{}
  \item Did you describe the limitations of your work?
    % \answerTODO{}
    \answerYes{See Section~\ref{sect:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
    % \answerTODO{}
    \answerYes{See Section~\ref{sect:limitation}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerTODO{}
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    % \answerTODO{}
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    % \answerTODO{}
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    % \answerTODO{}
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerTODO{}
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    % \answerTODO{}
    \answerYes{}
  \item Did you mention the license of the assets?
    % \answerTODO{}
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    % \answerTODO{}
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    % \answerTODO{}
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    % \answerTODO{}
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> inputs/experiments/5.1-experiment-setup.tex <==
\subsection{Experiment Setup}
\label{sect:setup}

\smallsection{Datasets}
In our experiments, we use two benchmark datasets: (1) {CIFAR-100}~\cite{Krizhevsky2009LearningML} consists of $50,000$ training samples from $100$ classes; and
(2) {Tiny-ImageNet}~\cite{TinyImageNet} is a miniature version of ImageNet~\cite{Deng2009ImageNetAL} consisting of $100,000$ training samples selected from $200$ classes. 
Due to computational constraints, we were not able to conduct experiments on ImageNet.
% Most of our experimental results are from CIFAR-100, and Tiny-ImageNet mainly serves as the second dataset to validate our claims.

\smallsection{Compared Methods}
We denote our novel student-oriented teacher network training framework as \emph{\ours}.
We compare \emph{\ours} with the common teacher training practice (\emph{i.e.}, Eq.~\ref{eq:empirical-risk}) in knowledge distillation (denoted as \emph{Standard}). 


\smallsection{Teacher-Student Pairs}
On CIFAR-100, we experiment with various network backbones including ResNet~\cite{He2016DeepRL}, Wide ResNet~\cite{Zagoruyko2016WideRN} and ShuffleNet~\cite{Zhang2018ShuffleNetAE, Tan2019MnasNetPN}. 
To test the applicability our method, we consider different aspects of model compression in knowledge distillation including reduction of the width or depth, and distillation between heterogeneous neural architectures. 
Due to space constraints, we select representative teacher-student pairs including WRN40-2/WRN40-1, WRN40-2/WRN16-2, 
% WRN40-2/ShuffleNetV2 
and ResNet32x4/ShuffleNetV2 to reflect all these aspects.
On Tiny-ImageNet, we conduct knowledge distillation between ResNet34 and ResNet18. 

\smallsection{Knowledge Distillation Algortihms}
We experiment with the original knowledge distillation method~({KD})~\cite{Hinton2015DistillingTK}, and a wide variety of other sophisticated knowledge distillation algorithms including {FitNets}~\cite{Romero2015FitNetsHF}, {AT}~\cite{Zagoruyko2017PayingMA}, {SP}~\cite{Tung2019SimilarityPreservingKD},
{CC}~\cite{Peng2019CorrelationCF},
{VID}~\cite{Ahn2019VariationalID}, {RKD}~\cite{Park2019RelationalKD}, {PKT}~\cite{Passalis2018LearningDR}, {AB}~\cite{Heo2019KnowledgeTV}, {FT}~\cite{Kim2018ParaphrasingCN},
{NST}~\cite{Huang2017LikeWY},
{CRD}~\cite{Tian2020ContrastiveRD}, {SSKD}~\cite{Xu2020KnowledgeDM} and 
% \textbf{OH}~\cite{Heo2019ACO} and 
{RCO}~\cite{Jin2019KnowledgeDV}. 
For the implementation of these algorithms, we refer to existing repositories for knowledge distillation~\cite{Tian2020ContrastiveRD, shah2020kdlib, matsubara2021torchdistill} and author-provided codes.

\jingbo{it's a bit weird to me if we mentioned all these KD algorithms but the Table 6 is actually in appendix? I wish to have Table 6 in the full paper if possible. }



\smallsection{Evaluation Metrics}
We report the teacher performance and the resulted student performance of the last teacher checkpoint.
The performance is always evaluated on the test set from 3 runs using different random seeds.
We present both mean and standard deviation of the test accuracy. For Tiny-ImageNet we also report the top-5 accuracy following the common setting.


% To demonstrate our \ours framework can guide the teacher training towards student generalization and mitigate the teacher ``overfitting'' problem, we report (1) the teacher test accuracy and the resulted student performance of the last teacher checkpoint (``\textbf{Last}''), which is available in practice; and (2) the teacher test accuracy and the resulted student performance of the ``best'' teacher checkpoint (``\textbf{Best}''). The ``best'' here refers to the one producing the highest student performance. 
% Note that the ``Best'' student performance is not achievable in practice.

% Due to the computational constraint, we didn't grid search all teacher checkpoints for the ``Best''. 
% Instead, we consider the checkpoints from the following three groups:
% (1) We select checkpoints along teacher's training trajectory every $10$ epochs and record the performance of the student distilled from them;
% (2) We also include the checkpoint with the best uncertainty measured by NLL, as the uncertainty on the test set (not necessarily available in practice) can sometimes indicate the best teacher~(see Section~\ref{sect:other-regularization});
% and (3) We further include the checkpoints around the first learning rate decay (e.g., epochs $150$ to $155$ on CIFAR-100), as Sec.~\ref{sect:other-regularization} shows that the best teacher often appears around this timing. 



\smallsection{Hyperparameter Settings}
For our teacher training method, we set $\lambda_{\text{CR}}^{\max} = 1$ for both datasets. For Lipschitz regularization, we set $\lambda_{\text{LR}} = 10^{-5}$ for CIFAR-100 and $\lambda_{\text{LR}} = 10^{-6}$ for Tiny-ImageNet, as the regularization term is the sum of the Lipschitz constants of trainable parameters, and the teacher model for Tiny-ImageNet has approximately $10$ times more parameters than that for CIFAR-100.
More detailed hyperparameter settings for neural network training and knowledge distillation algorithms can be found in Appendix~\ref{appendix:setting}.

